RAGEval: Scenario Specific RAG Evaluation Dataset Generation Framework

Retrieval-Augmented Generation (RAG) is a powerful approach that enables large language models (LLMs) to incorporate external knowledge. However, evaluating the effectiveness of RAG systems in specialized scenarios remains challenging due to the high costs of data construction and the lack of suitable evaluation metrics. This paper introduces RAGEval, a framework designed to assess RAG systems across diverse scenarios by generating high-quality documents, questions, answers, and references through a schema-based pipeline. With a focus on factual accuracy, we propose three novel metrics: Completeness, Hallucination, and Irrelevance to evaluate LLM generated responses rigorously. Experimental results show that RAGEval outperforms zero-shot and one-shot methods in terms of clarity, safety, conformity, and richness of generated samples. Furthermore, the use of LLMs for scoring the proposed metrics demonstrates a high level of consistency with human evaluations. RAGEval establishes a new paradigm for evaluating RAG systems in real-world applications. The code and dataset are released at https://github.com/OpenBMB/RAGEval.

==> sections/0_todo.tex <==
1. Figure1、Figure2 重绘 （罗逸凡、闫宇坤）
2. method部分要缩减，形成公式化的描述，文字部分进行总结，给出一个例子，然后着重进行概念抽象定义。
第一部分：给出一个问题的定义（说服别人，generation的pipeline是make sense的）；
第二部分：给出抽象的定义，schema、configuration、doc、q、a、r。
优先级最高：
第三部分：用说明+公式
（1）schema的定义，key分别是什么
（2）configuration的定义，key+value（定义成一个个fact {f}）
（3）document的generation（不谈细节，例如大纲，后面补一个，当文本非常负责时可以加一步outline
（4）d --> q、a
（5）d、q、a --> reference
（6）key-point 生成
把所有细节写在最后一段，包括outline、reference的refine等
3. 指标部分描述进行适当简化，公式不省略。开头一段写motivation
4. 数据质量评分简写结论，指标放到附录（人评部分不展开描述）
5. 不同domain的最优配置不一样？chunk-size之类的（罗逸凡）
6. limitation：
（1）伦理问题：safety相关的政策
（2）生成局限

10.15

1. 图表加上更丰富的信息描述
2. experiment部分确定相关模型都有cite
3. 整体过一遍grammaly 改语法错误
5. experiment部分新增实验+整体大改
6. refering to the appendix part

==> sections/3_method_backup.tex <==
\section{Method}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/progress.pdf}
    \caption{\ours{} Progress: \ding{192} summarizing a schema containing specific knowledge from seed documents. \ding{193} filling in factual information based on this schema to generate diverse configurations. \ding{194} generating documents according to the configurations. \ding{195} creating evaluation data composed of questions, answers, and references derived from the configurations and documents.}
    \label{fig:progress}
\end{figure*}

% Methodology (kunlun's thought)

% Todo:
% 1. abstract: add experiment results and our finding
% 2. add diverse domain results in the topk-chunk topk experiment
% 3. add ethical limitation part about the article generation
% 4. amend the methodology make it clear and easy to read


% Methodology
% In this section, we detail the methodology of our RAGEval framework, focusing on the rationale behind each step. This includes the dataset generation process, the QAR extraction method, the Dragonball dataset, and the evaluation metrics. Each method is designed to ensure a robust and comprehensive evaluation of large language models (LLMs) in domain-specific scenarios.

% 1. Seed Article Identification and Schema Definition
% Why: In order to generate realistic and relevant scenario-based articles, it's essential to first understand the structure and key information points of existing articles in the target domain.
% What We Do: We begin by identifying seed articles from the relevant domain. These articles serve as a foundation for understanding the typical structure and content of the domain.
% Purpose: From these seed articles, we extract a unique schema that captures the key elements (e.g., organizations, places, dates, events) specific to the article type. The schema provides a standardized template that ensures consistency and relevance in the generated articles. This step is crucial for maintaining domain specificity and ensuring that the generated content aligns with real-world structures.
% 2. Config Generation via Randomized Variables
% Why: To create a diverse dataset that can robustly evaluate LLMs, it's important to ensure variation in content while preserving structural consistency.
% What We Do: Based on the schema, we introduce random variables that allow us to populate the schema with specific content. This process generates multiple configurations for each article, where key elements like organizations, dates, and places are varied.
% Purpose: The purpose of this step is to ensure diversity while maintaining structural integrity. By varying key elements, we generate a broad range of scenarios that test the LLM's ability to adapt to different contexts. This ensures that the model is evaluated across a wide spectrum of domain-specific variations, avoiding overfitting to any single scenario.
% 3. Scenario Article Generation
% Why: Ensuring that the generated articles are coherent and contextually aligned with the given configs is critical for testing the LLM's ability to generate realistic and relevant content.
% What We Do: Using the configs and domain-specific instruction templates, we guide the LLM to generate target scenario articles. The articles are created with a focus on ensuring that the content is coherent, detailed, and consistent with the information in the configs.
% Purpose: This step ensures that the generated scenario articles are not only contextually accurate but also reflect the diversity introduced in the previous step. By aligning the generated content with the configs, we ensure that the model can produce detailed and domain-relevant articles that are consistent with real-world scenarios.
% 4. QAR Extraction Method
% Why: The ability to generate meaningful and accurate answers to domain-specific questions is a key measure of an LLM’s understanding and reasoning.
% What We Do: We implement a Question-Answer-Reference (QAR) extraction method. The LLM generates questions that are relevant to each scenario article, and then produces multiple answers from the content. These answers are compared to reference answers to ensure their accuracy and alignment.
% Purpose: The QAR extraction method is designed to evaluate the LLM's ability to reason over the generated content. By comparing the generated answers to reference answers, we measure the model’s ability to extract key information and provide accurate responses. This process helps identify both strengths and weaknesses in the model’s understanding of domain-specific scenarios.
% 5. Dragonball Dataset Details
% Why: A well-designed dataset is critical for evaluating the LLM's performance across different contexts and domains.
% What We Do: The Dragonball dataset is a synthetic dataset that we created specifically for the RAGEval framework. It includes a diverse set of scenario-based configurations, with varying organizations, places, dates, and events.
% Purpose: The Dragonball dataset is designed to stress-test the LLM’s ability to generate and evaluate answers in different contexts. By incorporating a wide range of domain-specific variations, the dataset ensures comprehensive coverage of different scenarios. This diversity helps assess the model's flexibility and robustness in handling various types of information.
% 6. Evaluation Metrics
% Why: A thorough evaluation requires multiple metrics to capture different aspects of model performance, such as accuracy, consistency, and diversity.


In this section, we elaborate on the proposed \ours{}. The overall generation process can be summarized as follows:

$\mathcal{S} \to \mathcal{C} \to \mathcal{D} \to (\mathcal{Q}, \mathcal{A}) \to \mathcal{R} \to \text{Keypoints}$

This sequence represents the flow from schema summary ($\mathcal{S}$) to configuration generation ($\mathcal{C}$), followed by document generation ($\mathcal{D}$). 
Question-answer pairs ($\mathcal{Q}, \mathcal{A}$) are then generated from the document, and relevant references ($\mathcal{R}$) are extracted to support the answers. 
Finally, keypoints are extracted to capture critical information from the answers.

\subsection{Schema Summary}

% In domain-specific scenarios, texts typically reflect specific knowledge,  corresponding to important factual information, such as clinical symptoms in medical contexts, regardless of stylistic differences. Taking a few documents as input, \ours{} captures such knowledge by summarizing a schema $\mathcal{S}$, which is later used to ensure the professionalism and reliability of the information in the subsequent document generation process like configs of the text. 

% Specifically, we utilized OpenAI’s GPT-4o for schema extraction and summarization. We generated an initial schema by submitting selected seed documents to GPTs and instructing them to incorporate domain-specific knowledge and focus areas. This schema was refined through iterative dialogues to ensure that the it was not only comprehensive but also sufficiently generalized to support diverse content generation tasks across various sub-domains. 
% To ensure diversity in the subsequent generated content, generalization of the schema is crucial. For instance, in the case of financial reports, the schema might encompass various industries ranging from agriculture to aviation. The fully developed schema includes key elements such as organizations, events, and dates. This approach ensures the diversity and scalability of subsequent generation tasks while minimizing the inclusion of specific elements that are unique to certain instances.

% In scenario-specific text generation, a schema $\mathcal{S}$ is defined as an abstract representation of key scenario-specific elements that capture essential factual knowledge types from input documents, such as clinical symptoms in medical contexts. The schema $\mathcal{S}$ serves as the backbone for content diversity and reliability in generation. This generalized structure enables consistent outputs in alignment with the professional contents across different scenarios.

In scenario-specific text generation, a schema $\mathcal{S}$ is defined as an abstract representation of key scenario-specific elements that encapsulate essential factual knowledge from input documents, such as clinical symptoms in medical contexts. The schema $\mathcal{S}$ serves as the backbone for ensuring content diversity and reliability in generation. This generalized structure enables consistent outputs that align with professional standards across different scenarios.


% We propose a method where, given a few seed documents, our model captures key scenario knowledge by summarizing the above schema $\mathcal{S}$. Specifically, we utilize GPTs for schema extraction and summarization. After generating an initial schema from selected seed documents. This schema $\mathcal{S}$ is then refined iteratively by experts familiar with the specific scenario and AI to make it comprehensive yet generalized enough to support content generation across sub-scenarios. For example, in financial reporting, the schema can span various industries like agriculture or aviation, covering elements like organizations, events, and dates. By generalizing the schema, our method supports diverse generation tasks, ensuring scalability while avoiding overly specific instance details. An example schema for the law scenario is provided in the appendix (see Figure \ref{fig:qar-schema-example}).

We propose a method in which, given a few seed documents, \ours{} captures key scenario knowledge by summarizing the schema $\mathcal{S}$. Specifically, we utilize GPTs for schema extraction and summarization. After generating an initial schema from selected seed documents, this schema $\mathcal{S}$ is iteratively refined by experts familiar with the specific scenario and GPT\footnote{The refining process can be found in the appendix ~\ref{appendix: schema_ref}.}, ensuring it is comprehensive and generalized enough to support content generation across sub-scenarios. For instance, in financial reporting, the schema can encompass various industries, such as agriculture or aviation, covering key elements like organizations, events, and dates. By generalizing the schema, our method supports diverse generation tasks, ensuring scalability while avoiding overly specific instance details. An example schema for the legal domain is provided in the appendix (see Figure \ref{fig:qar-schema-example}).

% This framework, represented by a schema $\mathcal{S}$, encapsulates the overall coverage of factual information in documents. The schema includes key elements such as organization, type, events, date, and place, summarizing the characteristic information of the scenario. To derive this schema, we employ LLMs to perform inductive reasoning based on a small set of seed texts. Although these seed texts may share the same type, they can vary greatly in style and specific factual content. For instance, financial reports might cover diverse industries from internet technology to food processing. This approach ensures the validity and comprehensiveness of the derived schema, enhancing the controllability of text generation and enabling the production of coherent, domain-appropriate content that aligns with the structural patterns of specific document types.


\subsection{Document Generation}

Generating scenario-specific documents with rich factual information and internal consistency is essential for effective dataset creation. To achieve this, we first generate configurations $\mathcal{C}$ derived from the schema $\mathcal{S}$ established in Stage 1. These configurations serve as references and constraints for text generation, ensuring consistency across different parts of the document.

Configurations $\mathcal{C}$ are generated using a hybrid approach that combines rule-based methods and LLMs to assign values to schema elements. Rule-based methods, including selecting values randomly from predefined options specified by scenario-specific knowledge, ensure high accuracy and factual consistency for structured data, while LLMs generate more complex or diverse content, providing a balance between consistency and creativity. For instance, in financial reports, configurations may include various sectors like ``agriculture'', ``aviation'', and ``construction'', covering multiple aspects of each domain. An example configuration for the law scenario is provided in the appendix (see Figure \ref{fig:qar-config-example}).

The document $\mathcal{D}$ is then generated by GPT-4o casting the factual information from configuration $\mathcal{C}$ into a structured narrative format appropriate for the specific scenario. For example, in medical records, the generated document may include categories like ``patient information'', ``medical history'', and "treatment plan" to ensure accuracy and relevance. In financial reports, we provide a summary of the company to maintain continuity and use different sections to cover ``Financial Report'', ``Corporate Governance'', and "Environmental and Social Responsibility."

% Generating virtual texts with rich factual information, logical coherence, and internal consistency is crucial for creating effective evaluation datasets. To achieve this, we first generate configurations $\mathcal{C}$ derived from the schema $\mathcal{S}$ established in Stage 1, rather than immediately producing the text. These configurations directly correspond to the types and content of factual information, serving as a reference and constraint for text generation. This approach ensures that information across different parts of the document remains more consistent with the configuration.

% To generate these configurations, we employ a hybrid approach combining rule-based and LLM-based methods to assign values to the schema elements. Rule-based value generation employs programmatic algorithms to create or select values, ensuring high accuracy, factual consistency, and efficiency, particularly for structured data like dates or categorical information. This approach is especially useful for schema elements with limited options or those requiring strict formatting. Complementing this, we leverage LLMs to generate more complex or diverse content. LLMs excel at creating varied and nuanced information, particularly for elements that require natural language understanding or creativity, such as detailed descriptions or complex relational information. This method allows us to produce a wide range of high-quality, diverse configurations. For instance, in the domain of financial reports, our configurations cover numerous sectors, including ``agriculture,'' ``aviation,'' and ``construction.'' In total, we have 20 different business domains in our documents. 

% Using the following strategy, we cast the factual information in a configuration $\mathcal{C}$ into a document $\mathcal{D}$: we integrate configuration details into a structured narrative format appropriate to the domain, incorporating domain-specific prior knowledge to ensure accuracy and contextual relevance. For medical records, this involves guidance on the structure and content, including categories of diseases, ensuring the inclusion of necessary fields such as ``patient information, medical history, examination results, diagnosis, treatment plan, and follow-up''. To mitigate hallucination issues in legal documents, the model only generates references to legal articles by their number, ensuring correct citations are added later. In financial reports, we provide a summary of the company to the model to ensure continuity. Financial documents often contain multiple chapters; thus, we use three sections: ``Financial Report, Corporate Governance, Environmental and Social Responsibility'' to cover various aspects. Given the complexity of financial events, we manually divide the configuration into the above three sections. We then provide these sections to GPT-4o to generate the relevant parts of the document. This prevents repeated overall summaries and maintains content flow. Finally, the three sections are concatenated to form a complete financial report.

\subsection{QRA Generation}

% \todo{Schema generation involves human expert based refinement, how does that impact the final quality of dataset. Is it necessary to refine schema, and what expertise is required for that? This could limit the scalability and reliability of the framework in new domains. Similarly document generation requires human experts. Authors need to provide full details of how many and what edits were made by human.}

In this subsection, we describe the process of generating Question-Reference-Answer (QRA) triples using the given documents $\mathcal{D}$ and configurations $\mathcal{C}$ to create an evaluation framework for information retrieval and reasoning. The goal is to ensure that generated content can be evaluated comprehensively across multiple aspects of information understanding.

\smallskip
\noindent
\textbf{Initializing QA Pairs.} We utilize configurations $\mathcal{C}$ to guide the generation of questions and initial answers. The configurations are embedded within prompts to ensure that generated questions are specific, and answers are precise. We address different types of questions, such as factual, multi-hop reasoning, summarization, and multi-document questions, aimed at evaluating various facets of language understanding. The GPT-4o model is provided with instructions and examples for each question type, resulting in targeted questions $\mathcal{Q}$ and initial answers $\mathcal{A}$. Specific prompts and examples are detailed in the appendix.

\smallskip
\noindent
\textbf{Extracting References.} Using the constructed questions $\mathcal{Q}$ and initial answers $\mathcal{A}$, we extract relevant information fragments (references) $\mathcal{R}$ from the documents $\mathcal{D}$. This is done using an extraction prompt that ensures the generated answers are grounded in the source material for reliability and traceability. Extracting these references enhances the comprehensiveness and consistency of the generated content.

\smallskip
\noindent
\textbf{Optimizing Answers and References.} To ensure alignment between answers $\mathcal{A}$ and references $\mathcal{R}$, we iteratively refine the answers. If references contain content missing from the answers, it is supplemented. Conversely, if the answers contain unsupported content, we either find the relevant references or remove the unsupported parts. This step reduces hallucinations and ensures that the final answers are accurate and well-supported by $\mathcal{R}$.

\smallskip
\noindent
\textbf{Generating Keypoints.} Keypoints are generated from answers $\mathcal{A}$ for each question $\mathcal{Q}$ to capture the critical information in responses. We employ a predefined prompt with in-context learning, including examples across different scenarios and question types. Typically, each response is distilled into 3-5 keypoints encompassing essential factual details, relevant inferences, and conclusions. This keypoint extraction supports a precise and reliable evaluation of generated content.


% \subsection{QRA Generation}

% In this subsection, we describe the process of generating Question-Reference-Answer (QRA) triples using the given documents $\mathcal{D}$ and configurations $\mathcal{C}$. The motivation behind this stage is to create a comprehensive evaluation framework that tests various aspects of information retrieval and reasoning capabilities.

% \smallskip
% \noindent
% \textbf{Initializing QA Pairs.} We leverage the configurations $\mathcal{C}$ to guide the generation of questions and initial answers. The configurations are embedded within the prompts to ensure that the generated questions are specific and the answers are precise. As shown in Table \ref{tab:question_type}, we address seven types of questions: factual questions, multi-hop reasoning questions, summarization questions, multi-document questions, and others. This diverse set of question types is designed to evaluate different facets of language understanding and information processing. The input to the GPT-4o model includes detailed instructions and a few examples for each question type, which are tailored according to the configurations. This results in questions $\mathcal{Q}$ and initial answers $\mathcal{A}$ that are more targeted and accurate. Specific prompts and examples are detailed in the appendices.

% \smallskip
% \noindent
% \textbf{Extracting References.} Our goal is to capture all pertinent references to support the answers comprehensively. Using the constructed questions $\mathcal{Q}$ and initial answers $\mathcal{A}$, we extract relevant information fragments (references) $\mathcal{R}$ from the articles by utilizing an extracting prompt given the relative documents. In the prompt, we emphasize the importance of grounding answers in the source material to ensure reliability and traceability. This step enhances the comprehensiveness and accuracy of the answers by ensuring they are well-supported by the source documents. 
% % The constraints and rules applied during this extraction phase ensure that the references are relevant and directly support the answers, leading to more precise and comprehensive QRA triples.

% \smallskip
% \noindent
% \textbf{Optimizing Answers and References.} Optimizing answers is crucial to ensure accuracy and alignment with the provided references $\mathcal{R}$, thereby minimizing misinformation and enhancing the reliability of the generated content. The refinement process follows these principles: If the references $\mathcal{R}$ contain content not present in the initial answers $\mathcal{A}$, we supplement the answers accordingly. Conversely, if the initial answers $\mathcal{A}$ contain content not found in the references $\mathcal{R}$, we first check the article for any overlooked references. If such references are found, we add them to the reference set and keep the answer unchanged. If no corresponding references are found, we remove the irrelevant content from the answer. This approach addresses the issue of hallucinations that may arise during the answer generation process, ensuring that the final answers are both accurate and well-supported by the references $\mathcal{R}$.

% \smallskip
% \noindent
% \textbf{Generating Keypoints.} In our evaluation framework, assessing answers is not merely about correctness or keyword matching but about identifying the critical information contained in the responses. To facilitate this, we generate keypoints from the standard answers $\mathcal{A}$ for each question $\mathcal{Q}$.To generate these keypoints, we employ a predefined prompt for the GPT-4o model, which supports both Chinese and English. The prompt is designed using in-context learning, providing examples of keypoint extraction across different domains and question types. This includes cases where the answer is unanswerable, and the keypoints reflect that appropriately. Typically, responses are distilled into 3-5 keypoints, encompassing indispensable factual information, relevant inferences, and final conclusions necessary to answer the question.By extracting these keypoints, we ensure that our evaluation is grounded in clearly defined and relevant information, enhancing the precision and reliability of the subsequent metrics calculation.

\subsection{DragonBall Dataset}
Leveraging the generation method mentioned above, we construct the DragonBall dataset, which stands for \textbf{D}iverse \textbf{RAG} \textbf{O}m\textbf{n}i-\textbf{B}enchmark for \textbf{All} scenarios. This dataset encompasses a wide array of texts and related RAG questions across three critical scenarios: finance, law, and medical. Moreover, the dataset includes both Chinese and English texts, providing a comprehensive resource for multilingual and scenario-specific research. In total, we have 6711 questions in our dataset. More details on the generated Dragonball dataset can be found in the appendix \ref{sec:verfication}, \ref{dragonball}, including the human evaluations about the quality of the generated data.

% For document generation, the dataset includes texts from 20 different corporate domains in finance, with one randomly selected text per domain; 10 different legal domains, with two randomly selected texts per domain; and 19 major medical categories, each with two subcategories and one randomly selected text per major category. This ensures a balanced number of human-evaluated documents across finance, law, and medical domains.


% In Table \ref{tab:dataset_stats}, we present a detailed breakdown of the DRAGONBall dataset. The first section of the table shows the distribution of documents across the three domains (finance, legal, and medical) in both Chinese (CN) and English (EN), with an equal number of documents for each language. The second section categorizes the types of questions included in the dataset, providing percentages for each type. The third section details the distribution of the number of reference documents used in answering the questions, reflecting the complexity and variability of the dataset. In total, the dataset comprises 6711 questions.

% To ensure the high quality of the QRA triples, we first consider the balance and diversity among the different question types, and then we remove homogeneous and meaningless questions. For example, if the number of unanswerable questions is insufficient, we supplement them according to the article. Second, we eliminate redundant references and answer statements and correct logical reasoning errors in the answers to ensure the dataset quality.

    
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/question_type_distribution.pdf}
    
%     \caption{Distribution of question type.}
%     \label{fig:question_type_distribution}
% \end{figure}
% \vspace{0.5cm}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/reference_distribution.pdf}
%     \caption{Distribution of reference.}
%     \label{fig:reference_distribution}
% \end{figure}
% \vspace{0.5cm}



\subsection{Evaluation Metrics for RAG Systems}



In this work, we propose a comprehensive evaluation framework for RAG systems, considering both retrieval and generation components.

We define multiple metrics to evaluate the model's effectiveness and efficiency in the retrieval phase. These metrics are designed explicitly for RAG systems, considering the situations when generating with incomplete and noisy information.

\subsubsection{Retrieval Metrics}

\paragraph{Recall.} We introduce the RAG Retrieval Recall metric to evaluate the effectiveness of the retrieval process in matching ground truth references. The Recall is formally defined as
\begin{equation}
\small
    \text{Recall} = \frac{1}{n} \sum_{i=1}^{n} \mathbbm{1}(M(G_i, \mathcal{R})),
    \label{eq:recall}
\end{equation}
where $n$ is the total number of ground truth references, $G_i$ denotes the $i$-th ground truth reference, $\mathcal{R} = \{R_1, R_2, \ldots, R_k\}$ represents the set of retrieved references, $M(G_i, \mathcal{R})$ is a boolean function that returns true if all sentences in $G_i$ are found in at least one reference in $\mathcal{R}$, and false otherwise, and $\mathbbm{1}(\cdot)$ is the indicator function, returning 1 if the condition is true and 0 otherwise.

This metric assesses the alignment between retrieved and ground truth references at the sentence level. A ground truth reference is considered successfully recalled if all its constituent sentences are present in at least one of the retrieved references.

\paragraph{Effective Information Rate (EIR).} This metric quantifies the proportion of relevant information within the retrieved passages, ensuring that the retrieval process is both accurate and efficient in terms of information content. It is calculated as
\begin{equation}
\small
    \text{EIR} = \frac{\sum_{i=1}^{m} |G_i \cap R_t|}{\sum_{j=1}^{k} |R_j|},
\end{equation}
where $G_i$ is the $i$-th ground truth reference, $R_t$ is the set of total retrieved passages, $m$ is the number of ground truth references successfully matched, $|G_i \cap R_t|$ represents the number of words in the intersection of the $i$-th ground truth reference and the concatenated retrieved passages $R_t$, calculated only if $G_i$ is matched in $R_t$, $|R_j|$ represents the total number of words in the $j$-th retrieved passage, and $k$ is the total number of retrieved passages.

To calculate $|G_i \cap R_t|$ at the sentence level, follow these steps: 1) divide $G_i$ into individual sentences, 2) for each sentence in $G_i$, check if it matches any sentence in $R_t$, 3) calculate the number of words in the matched sentences, and 4) sum the number of words from all matched sentences to get $|G_i \cap R_t|$. This ensures that the overlap is calculated based on sentence-level matches, providing a more granular and accurate measure of relevant information within the retrieved passages.

\subsubsection{Generation Metrics}

For the generation component, we introduce novel metrics tailored for RAG evaluation. These metrics provide a comprehensive evaluation of the quality and reliability of generated answers.

\paragraph{Completeness.} Completeness measures how well the generated answer captures the key information from the ground truth. We employ a large language model (LLM) to generate a set of key points $K = \{k_1, k_2, \ldots, k_n\}$ from the ground truth. The Completeness score is then calculated as the proportion of key points semantically covered by the generated answer $A$:
\begin{equation}
\small
    \text{Comp}(A, K) = \frac{1}{|K|} \sum_{i=1}^{n} \mathbbm{1}[A \text{ covers } k_i],
\end{equation}
where $\mathbbm{1}[\cdot]$ is an indicator function that evaluates to 1 if the generated answer $A$ semantically covers the key point $k_i$, and 0 otherwise. Here, ``covers'' means that the generated answer contains information consistent with and correctly representing the key point. Specifically, for a key point to be considered covered, the generated answer must not only include the relevant information but also present it accurately without contradictions or factual errors.

\paragraph{Hallucination.} Hallucination identifies instances where the content contradicts key points, highlighting potential inaccuracies. The Hallucination score is calculated as
\begin{equation}
\small
    \text{Hallu}(A, K) = \frac{1}{|K|} \sum_{i=1}^{n} \mathbbm{1}[A \text{ contradicts } k_i],
\end{equation}
where $\mathbbm{1}[\cdot]$ is an indicator function that evaluates to 1 if the generated answer $A$ contradicts the key point $k_i$, and 0 otherwise.

\paragraph{Irrelevancy.} Irrelevancy assesses the proportion of key points from the ground truth that are neither covered nor contradicted by the generated answer. Irrelevancy quantifies the proportion of key points neither covered nor contradicted, indicating areas where the answer fails to engage with relevant information. The Irrelevancy score is calculated as
\begin{equation}
\small
    \text{Irr}(A, K) = 1 - \text{Comp}(A, K) - \text{Hallu}(A, K).
\end{equation}

These metrics—Completeness, Hallucination, and Irrelevancy—together pinpoint specific strengths and weaknesses of RAG models, ensuring generated answers are informative, accurate, and relevant, thereby enhancing their overall quality and trustworthiness.
